P3LS: Point Process Partial Least Squares

Many studies collect data that can be considered as a realization of a point process. Included are medical imaging data where photon counts are recorded by a gamma camera from patients being injected with a gamma emitting tracer. It is of interest to develop analytic methods that can help with diagnosis as well as in the training of inexpert radiologists. Partial least squares (PLS) is a popular analytic approach that combines features from linear modeling as well as dimension reduction to provide parsimonious prediction and classification. However, existing PLS methodologies do not include the analysis of point process predictors. In this article, we introduce point process PLS (P3LS) for analyzing latent time-varying intensity functions from collections of inhomogeneous point processes. A novel estimation procedure for $P^3LS$ is developed that utilizes the properties of log-Gaussian Cox processes, and its empirical properties are examined in simulation studies. The method is used to analyze kidney functionality in patients with renal disease in order to aid in the diagnosis of kidney obstruction.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}






==> rgbbeamer.tex <==
\xdefinecolor{AliceBlue}{rgb}{0.94,0.97,1.00}
\xdefinecolor{AntiqueWhite1}{rgb}{1.00,0.94,0.86}
\xdefinecolor{AntiqueWhite2}{rgb}{0.93,0.87,0.80}
\xdefinecolor{AntiqueWhite3}{rgb}{0.80,0.75,0.69}
\xdefinecolor{AntiqueWhite4}{rgb}{0.55,0.51,0.47}
\xdefinecolor{AntiqueWhite}{rgb}{0.98,0.92,0.84}
\xdefinecolor{BlanchedAlmond}{rgb}{1.00,0.92,0.80}
\xdefinecolor{BlueViolet}{rgb}{0.54,0.17,0.89}
\xdefinecolor{CadetBlue1}{rgb}{0.60,0.96,1.00}
\xdefinecolor{CadetBlue2}{rgb}{0.56,0.90,0.93}
\xdefinecolor{CadetBlue3}{rgb}{0.48,0.77,0.80}
\xdefinecolor{CadetBlue4}{rgb}{0.33,0.53,0.55}
\xdefinecolor{CadetBlue}{rgb}{0.37,0.62,0.63}
\xdefinecolor{CornflowerBlue}{rgb}{0.39,0.58,0.93}
\xdefinecolor{DarkBlue}{rgb}{0.00,0.00,0.55}
\xdefinecolor{DarkCyan}{rgb}{0.00,0.55,0.55}
\xdefinecolor{DarkGoldenrod1}{rgb}{1.00,0.73,0.06}
\xdefinecolor{DarkGoldenrod2}{rgb}{0.93,0.68,0.05}
\xdefinecolor{DarkGoldenrod3}{rgb}{0.80,0.58,0.05}
\xdefinecolor{DarkGoldenrod4}{rgb}{0.55,0.40,0.03}
\xdefinecolor{DarkGoldenrod}{rgb}{0.72,0.53,0.04}
\xdefinecolor{DarkGray}{rgb}{0.66,0.66,0.66}
\xdefinecolor{DarkGreen}{rgb}{0.00,0.39,0.00}
\xdefinecolor{DarkGrey}{rgb}{0.66,0.66,0.66}
\xdefinecolor{DarkKhaki}{rgb}{0.74,0.72,0.42}
\xdefinecolor{DarkMagenta}{rgb}{0.55,0.00,0.55}
\xdefinecolor{DarkOliveGreen1}{rgb}{0.79,1.00,0.44}
\xdefinecolor{DarkOliveGreen2}{rgb}{0.74,0.93,0.41}
\xdefinecolor{DarkOliveGreen3}{rgb}{0.64,0.80,0.35}
\xdefinecolor{DarkOliveGreen4}{rgb}{0.43,0.55,0.24}
\xdefinecolor{DarkOliveGreen}{rgb}{0.33,0.42,0.18}
\xdefinecolor{DarkOrange1}{rgb}{1.00,0.50,0.00}
\xdefinecolor{DarkOrange2}{rgb}{0.93,0.46,0.00}
\xdefinecolor{DarkOrange3}{rgb}{0.80,0.40,0.00}
\xdefinecolor{DarkOrange4}{rgb}{0.55,0.27,0.00}
\xdefinecolor{DarkOrange}{rgb}{1.00,0.55,0.00}
\xdefinecolor{DarkOrchid1}{rgb}{0.75,0.24,1.00}
\xdefinecolor{DarkOrchid2}{rgb}{0.70,0.23,0.93}
\xdefinecolor{DarkOrchid3}{rgb}{0.60,0.20,0.80}
\xdefinecolor{DarkOrchid4}{rgb}{0.41,0.13,0.55}
\xdefinecolor{DarkOrchid}{rgb}{0.60,0.20,0.80}
\xdefinecolor{DarkRed}{rgb}{0.55,0.00,0.00}
\xdefinecolor{DarkSalmon}{rgb}{0.91,0.59,0.48}
\xdefinecolor{DarkSeaGreen1}{rgb}{0.76,1.00,0.76}
\xdefinecolor{DarkSeaGreen2}{rgb}{0.71,0.93,0.71}
\xdefinecolor{DarkSeaGreen3}{rgb}{0.61,0.80,0.61}
\xdefinecolor{DarkSeaGreen4}{rgb}{0.41,0.55,0.41}
\xdefinecolor{DarkSeaGreen}{rgb}{0.56,0.74,0.56}
\xdefinecolor{DarkSlateBlue}{rgb}{0.28,0.24,0.55}
\xdefinecolor{DarkSlateGray1}{rgb}{0.59,1.00,1.00}
\xdefinecolor{DarkSlateGray2}{rgb}{0.55,0.93,0.93}
\xdefinecolor{DarkSlateGray3}{rgb}{0.47,0.80,0.80}
\xdefinecolor{DarkSlateGray4}{rgb}{0.32,0.55,0.55}
\xdefinecolor{DarkSlateGray}{rgb}{0.18,0.31,0.31}
\xdefinecolor{DarkSlateGrey}{rgb}{0.18,0.31,0.31}
\xdefinecolor{DarkTurquoise}{rgb}{0.00,0.81,0.82}
\xdefinecolor{DarkViolet}{rgb}{0.58,0.00,0.83}
\xdefinecolor{DeepPink1}{rgb}{1.00,0.08,0.58}
\xdefinecolor{DeepPink2}{rgb}{0.93,0.07,0.54}
\xdefinecolor{DeepPink3}{rgb}{0.80,0.06,0.46}
\xdefinecolor{DeepPink4}{rgb}{0.55,0.04,0.31}
\xdefinecolor{DeepPink}{rgb}{1.00,0.08,0.58}
\xdefinecolor{DeepSkyBlue1}{rgb}{0.00,0.75,1.00}
\xdefinecolor{DeepSkyBlue2}{rgb}{0.00,0.70,0.93}
\xdefinecolor{DeepSkyBlue3}{rgb}{0.00,0.60,0.80}
\xdefinecolor{DeepSkyBlue4}{rgb}{0.00,0.41,0.55}
\xdefinecolor{DeepSkyBlue}{rgb}{0.00,0.75,1.00}
\xdefinecolor{DimGray}{rgb}{0.41,0.41,0.41}
\xdefinecolor{DimGrey}{rgb}{0.41,0.41,0.41}
\xdefinecolor{DodgerBlue1}{rgb}{0.12,0.56,1.00}
\xdefinecolor{DodgerBlue2}{rgb}{0.11,0.53,0.93}
\xdefinecolor{DodgerBlue3}{rgb}{0.09,0.45,0.80}
\xdefinecolor{DodgerBlue4}{rgb}{0.06,0.31,0.55}
\xdefinecolor{DodgerBlue}{rgb}{0.12,0.56,1.00}
\xdefinecolor{FloralWhite}{rgb}{1.00,0.98,0.94}
\xdefinecolor{ForestGreen}{rgb}{0.13,0.55,0.13}
\xdefinecolor{GhostWhite}{rgb}{0.97,0.97,1.00}
\xdefinecolor{GreenYellow}{rgb}{0.68,1.00,0.18}
\xdefinecolor{HotPink1}{rgb}{1.00,0.43,0.71}
\xdefinecolor{HotPink2}{rgb}{0.93,0.42,0.65}
\xdefinecolor{HotPink3}{rgb}{0.80,0.38,0.56}
\xdefinecolor{HotPink4}{rgb}{0.55,0.23,0.38}
\xdefinecolor{HotPink}{rgb}{1.00,0.41,0.71}
\xdefinecolor{IndianRed1}{rgb}{1.00,0.42,0.42}
\xdefinecolor{IndianRed2}{rgb}{0.93,0.39,0.39}
\xdefinecolor{IndianRed3}{rgb}{0.80,0.33,0.33}
\xdefinecolor{IndianRed4}{rgb}{0.55,0.23,0.23}
\xdefinecolor{IndianRed}{rgb}{0.80,0.36,0.36}
\xdefinecolor{LavenderBlush1}{rgb}{1.00,0.94,0.96}
\xdefinecolor{LavenderBlush2}{rgb}{0.93,0.88,0.90}
\xdefinecolor{LavenderBlush3}{rgb}{0.80,0.76,0.77}
\xdefinecolor{LavenderBlush4}{rgb}{0.55,0.51,0.53}
\xdefinecolor{LavenderBlush}{rgb}{1.00,0.94,0.96}
\xdefinecolor{LawnGreen}{rgb}{0.49,0.99,0.00}
\xdefinecolor{LemonChiffon1}{rgb}{1.00,0.98,0.80}
\xdefinecolor{LemonChiffon2}{rgb}{0.93,0.91,0.75}
\xdefinecolor{LemonChiffon3}{rgb}{0.80,0.79,0.65}
\xdefinecolor{LemonChiffon4}{rgb}{0.55,0.54,0.44}
\xdefinecolor{LemonChiffon}{rgb}{1.00,0.98,0.80}
\xdefinecolor{LightBlue1}{rgb}{0.75,0.94,1.00}
\xdefinecolor{LightBlue2}{rgb}{0.70,0.87,0.93}
\xdefinecolor{LightBlue3}{rgb}{0.60,0.75,0.80}
\xdefinecolor{LightBlue4}{rgb}{0.41,0.51,0.55}
\xdefinecolor{LightBlue}{rgb}{0.68,0.85,0.90}
\xdefinecolor{LightCoral}{rgb}{0.94,0.50,0.50}
\xdefinecolor{LightCyan1}{rgb}{0.88,1.00,1.00}
\xdefinecolor{LightCyan2}{rgb}{0.82,0.93,0.93}
\xdefinecolor{LightCyan3}{rgb}{0.71,0.80,0.80}
\xdefinecolor{LightCyan4}{rgb}{0.48,0.55,0.55}
\xdefinecolor{LightCyan}{rgb}{0.88,1.00,1.00}
\xdefinecolor{LightGoldenrod1}{rgb}{1.00,0.93,0.55}
\xdefinecolor{LightGoldenrod2}{rgb}{0.93,0.86,0.51}
\xdefinecolor{LightGoldenrod3}{rgb}{0.80,0.75,0.44}
\xdefinecolor{LightGoldenrod4}{rgb}{0.55,0.51,0.30}
\xdefinecolor{LightGoldenrodYellow}{rgb}{0.98,0.98,0.82}
\xdefinecolor{LightGoldenrod}{rgb}{0.93,0.87,0.51}
\xdefinecolor{LightGray}{rgb}{0.83,0.83,0.83}
\xdefinecolor{LightGreen}{rgb}{0.56,0.93,0.56}
\xdefinecolor{LightGrey}{rgb}{0.83,0.83,0.83}
\xdefinecolor{LightPink1}{rgb}{1.00,0.68,0.73}
\xdefinecolor{LightPink2}{rgb}{0.93,0.64,0.68}
\xdefinecolor{LightPink3}{rgb}{0.80,0.55,0.58}
\xdefinecolor{LightPink4}{rgb}{0.55,0.37,0.40}
\xdefinecolor{LightPink}{rgb}{1.00,0.71,0.76}
\xdefinecolor{LightSalmon1}{rgb}{1.00,0.63,0.48}
\xdefinecolor{LightSalmon2}{rgb}{0.93,0.58,0.45}
\xdefinecolor{LightSalmon3}{rgb}{0.80,0.51,0.38}
\xdefinecolor{LightSalmon4}{rgb}{0.55,0.34,0.26}
\xdefinecolor{LightSalmon}{rgb}{1.00,0.63,0.48}
\xdefinecolor{LightSeaGreen}{rgb}{0.13,0.70,0.67}
\xdefinecolor{LightSkyBlue1}{rgb}{0.69,0.89,1.00}
\xdefinecolor{LightSkyBlue2}{rgb}{0.64,0.83,0.93}
\xdefinecolor{LightSkyBlue3}{rgb}{0.55,0.71,0.80}
\xdefinecolor{LightSkyBlue4}{rgb}{0.38,0.48,0.55}
\xdefinecolor{LightSkyBlue}{rgb}{0.53,0.81,0.98}
\xdefinecolor{LightSlateBlue}{rgb}{0.52,0.44,1.00}
\xdefinecolor{LightSlateGray}{rgb}{0.47,0.53,0.60}
\xdefinecolor{LightSlateGrey}{rgb}{0.47,0.53,0.60}
\xdefinecolor{LightSteelBlue1}{rgb}{0.79,0.88,1.00}
\xdefinecolor{LightSteelBlue2}{rgb}{0.74,0.82,0.93}
\xdefinecolor{LightSteelBlue3}{rgb}{0.64,0.71,0.80}
\xdefinecolor{LightSteelBlue4}{rgb}{0.43,0.48,0.55}
\xdefinecolor{LightSteelBlue}{rgb}{0.69,0.77,0.87}
\xdefinecolor{LightYellow1}{rgb}{1.00,1.00,0.88}
\xdefinecolor{LightYellow2}{rgb}{0.93,0.93,0.82}
\xdefinecolor{LightYellow3}{rgb}{0.80,0.80,0.71}
\xdefinecolor{LightYellow4}{rgb}{0.55,0.55,0.48}
\xdefinecolor{LightYellow}{rgb}{1.00,1.00,0.88}
\xdefinecolor{LimeGreen}{rgb}{0.20,0.80,0.20}
\xdefinecolor{MediumAquamarine}{rgb}{0.40,0.80,0.67}
\xdefinecolor{MediumBlue}{rgb}{0.00,0.00,0.80}
\xdefinecolor{MediumOrchid1}{rgb}{0.88,0.40,1.00}
\xdefinecolor{MediumOrchid2}{rgb}{0.82,0.37,0.93}
\xdefinecolor{MediumOrchid3}{rgb}{0.71,0.32,0.80}
\xdefinecolor{MediumOrchid4}{rgb}{0.48,0.22,0.55}
\xdefinecolor{MediumOrchid}{rgb}{0.73,0.33,0.83}
\xdefinecolor{MediumPurple1}{rgb}{0.67,0.51,1.00}
\xdefinecolor{MediumPurple2}{rgb}{0.62,0.47,0.93}
\xdefinecolor{MediumPurple3}{rgb}{0.54,0.41,0.80}
\xdefinecolor{MediumPurple4}{rgb}{0.36,0.28,0.55}
\xdefinecolor{MediumPurple}{rgb}{0.58,0.44,0.86}
\xdefinecolor{MediumSeaGreen}{rgb}{0.24,0.70,0.44}
\xdefinecolor{MediumSlateBlue}{rgb}{0.48,0.41,0.93}
\xdefinecolor{MediumSpringGreen}{rgb}{0.00,0.98,0.60}
\xdefinecolor{MediumTurquoise}{rgb}{0.28,0.82,0.80}
\xdefinecolor{MediumVioletRed}{rgb}{0.78,0.08,0.52}
\xdefinecolor{MidnightBlue}{rgb}{0.10,0.10,0.44}
\xdefinecolor{MintCream}{rgb}{0.96,1.00,0.98}
\xdefinecolor{MistyRose1}{rgb}{1.00,0.89,0.88}
\xdefinecolor{MistyRose2}{rgb}{0.93,0.84,0.82}
\xdefinecolor{MistyRose3}{rgb}{0.80,0.72,0.71}
\xdefinecolor{MistyRose4}{rgb}{0.55,0.49,0.48}
\xdefinecolor{MistyRose}{rgb}{1.00,0.89,0.88}
\xdefinecolor{NavajoWhite1}{rgb}{1.00,0.87,0.68}
\xdefinecolor{NavajoWhite2}{rgb}{0.93,0.81,0.63}
\xdefinecolor{NavajoWhite3}{rgb}{0.80,0.70,0.55}
\xdefinecolor{NavajoWhite4}{rgb}{0.55,0.47,0.37}
\xdefinecolor{NavajoWhite}{rgb}{1.00,0.87,0.68}
\xdefinecolor{NavyBlue}{rgb}{0.00,0.00,0.50}
\xdefinecolor{OldLace}{rgb}{0.99,0.96,0.90}
\xdefinecolor{OliveDrab1}{rgb}{0.75,1.00,0.24}
\xdefinecolor{OliveDrab2}{rgb}{0.70,0.93,0.23}
\xdefinecolor{OliveDrab3}{rgb}{0.60,0.80,0.20}
\xdefinecolor{OliveDrab4}{rgb}{0.41,0.55,0.13}
\xdefinecolor{OliveDrab}{rgb}{0.42,0.56,0.14}
\xdefinecolor{OrangeRed1}{rgb}{1.00,0.27,0.00}
\xdefinecolor{OrangeRed2}{rgb}{0.93,0.25,0.00}
\xdefinecolor{OrangeRed3}{rgb}{0.80,0.22,0.00}
\xdefinecolor{OrangeRed4}{rgb}{0.55,0.15,0.00}
\xdefinecolor{OrangeRed}{rgb}{1.00,0.27,0.00}
\xdefinecolor{PaleGoldenrod}{rgb}{0.93,0.91,0.67}
\xdefinecolor{PaleGreen1}{rgb}{0.60,1.00,0.60}
\xdefinecolor{PaleGreen2}{rgb}{0.56,0.93,0.56}
\xdefinecolor{PaleGreen3}{rgb}{0.49,0.80,0.49}
\xdefinecolor{PaleGreen4}{rgb}{0.33,0.55,0.33}
\xdefinecolor{PaleGreen}{rgb}{0.60,0.98,0.60}
\xdefinecolor{PaleTurquoise1}{rgb}{0.73,1.00,1.00}
\xdefinecolor{PaleTurquoise2}{rgb}{0.68,0.93,0.93}
\xdefinecolor{PaleTurquoise3}{rgb}{0.59,0.80,0.80}
\xdefinecolor{PaleTurquoise4}{rgb}{0.40,0.55,0.55}
\xdefinecolor{PaleTurquoise}{rgb}{0.69,0.93,0.93}
\xdefinecolor{PaleVioletRed1}{rgb}{1.00,0.51,0.67}
\xdefinecolor{PaleVioletRed2}{rgb}{0.93,0.47,0.62}
\xdefinecolor{PaleVioletRed3}{rgb}{0.80,0.41,0.54}
\xdefinecolor{PaleVioletRed4}{rgb}{0.55,0.28,0.36}
\xdefinecolor{PaleVioletRed}{rgb}{0.86,0.44,0.58}
\xdefinecolor{PapayaWhip}{rgb}{1.00,0.94,0.84}
\xdefinecolor{PeachPuff1}{rgb}{1.00,0.85,0.73}
\xdefinecolor{PeachPuff2}{rgb}{0.93,0.80,0.68}
\xdefinecolor{PeachPuff3}{rgb}{0.80,0.69,0.58}
\xdefinecolor{PeachPuff4}{rgb}{0.55,0.47,0.40}
\xdefinecolor{PeachPuff}{rgb}{1.00,0.85,0.73}
\xdefinecolor{PowderBlue}{rgb}{0.69,0.88,0.90}
\xdefinecolor{RosyBrown1}{rgb}{1.00,0.76,0.76}
\xdefinecolor{RosyBrown2}{rgb}{0.93,0.71,0.71}
\xdefinecolor{RosyBrown3}{rgb}{0.80,0.61,0.61}
\xdefinecolor{RosyBrown4}{rgb}{0.55,0.41,0.41}
\xdefinecolor{RosyBrown}{rgb}{0.74,0.56,0.56}
\xdefinecolor{RoyalBlue1}{rgb}{0.28,0.46,1.00}
\xdefinecolor{RoyalBlue2}{rgb}{0.26,0.43,0.93}
\xdefinecolor{RoyalBlue3}{rgb}{0.23,0.37,0.80}
\xdefinecolor{RoyalBlue4}{rgb}{0.15,0.25,0.55}
\xdefinecolor{RoyalBlue}{rgb}{0.25,0.41,0.88}
\xdefinecolor{SaddleBrown}{rgb}{0.55,0.27,0.07}
\xdefinecolor{SandyBrown}{rgb}{0.96,0.64,0.38}
\xdefinecolor{SeaGreen1}{rgb}{0.33,1.00,0.62}
\xdefinecolor{SeaGreen2}{rgb}{0.31,0.93,0.58}
\xdefinecolor{SeaGreen3}{rgb}{0.26,0.80,0.50}
\xdefinecolor{SeaGreen4}{rgb}{0.18,0.55,0.34}
\xdefinecolor{SeaGreen}{rgb}{0.18,0.55,0.34}
\xdefinecolor{SkyBlue1}{rgb}{0.53,0.81,1.00}
\xdefinecolor{SkyBlue2}{rgb}{0.49,0.75,0.93}
\xdefinecolor{SkyBlue3}{rgb}{0.42,0.65,0.80}
\xdefinecolor{SkyBlue4}{rgb}{0.29,0.44,0.55}
\xdefinecolor{SkyBlue}{rgb}{0.53,0.81,0.92}
\xdefinecolor{SlateBlue1}{rgb}{0.51,0.44,1.00}
\xdefinecolor{SlateBlue2}{rgb}{0.48,0.40,0.93}
\xdefinecolor{SlateBlue3}{rgb}{0.41,0.35,0.80}
\xdefinecolor{SlateBlue4}{rgb}{0.28,0.24,0.55}
\xdefinecolor{SlateBlue}{rgb}{0.42,0.35,0.80}
\xdefinecolor{SlateGray1}{rgb}{0.78,0.89,1.00}
\xdefinecolor{SlateGray2}{rgb}{0.73,0.83,0.93}
\xdefinecolor{SlateGray3}{rgb}{0.62,0.71,0.80}
\xdefinecolor{SlateGray4}{rgb}{0.42,0.48,0.55}
\xdefinecolor{SlateGray}{rgb}{0.44,0.50,0.56}
\xdefinecolor{SlateGrey}{rgb}{0.44,0.50,0.56}
\xdefinecolor{SpringGreen1}{rgb}{0.00,1.00,0.50}
\xdefinecolor{SpringGreen2}{rgb}{0.00,0.93,0.46}
\xdefinecolor{SpringGreen3}{rgb}{0.00,0.80,0.40}
\xdefinecolor{SpringGreen4}{rgb}{0.00,0.55,0.27}
\xdefinecolor{SpringGreen}{rgb}{0.00,1.00,0.50}
\xdefinecolor{SteelBlue1}{rgb}{0.39,0.72,1.00}
\xdefinecolor{SteelBlue2}{rgb}{0.36,0.67,0.93}
\xdefinecolor{SteelBlue3}{rgb}{0.31,0.58,0.80}
\xdefinecolor{SteelBlue4}{rgb}{0.21,0.39,0.55}
\xdefinecolor{SteelBlue}{rgb}{0.27,0.51,0.71}
\xdefinecolor{VioletRed1}{rgb}{1.00,0.24,0.59}
\xdefinecolor{VioletRed2}{rgb}{0.93,0.23,0.55}
\xdefinecolor{VioletRed3}{rgb}{0.80,0.20,0.47}
\xdefinecolor{VioletRed4}{rgb}{0.55,0.13,0.32}
\xdefinecolor{VioletRed}{rgb}{0.82,0.13,0.56}
\xdefinecolor{WhiteSmoke}{rgb}{0.96,0.96,0.96}
\xdefinecolor{YellowGreen}{rgb}{0.60,0.80,0.20}
\xdefinecolor{aliceblue}{rgb}{0.94,0.97,1.00}
\xdefinecolor{antiquewhite}{rgb}{0.98,0.92,0.84}
\xdefinecolor{aquamarine1}{rgb}{0.50,1.00,0.83}
\xdefinecolor{aquamarine2}{rgb}{0.46,0.93,0.78}
\xdefinecolor{aquamarine3}{rgb}{0.40,0.80,0.67}
\xdefinecolor{aquamarine4}{rgb}{0.27,0.55,0.45}
\xdefinecolor{aquamarine}{rgb}{0.50,1.00,0.83}
\xdefinecolor{azure1}{rgb}{0.94,1.00,1.00}
\xdefinecolor{azure2}{rgb}{0.88,0.93,0.93}
\xdefinecolor{azure3}{rgb}{0.76,0.80,0.80}
\xdefinecolor{azure4}{rgb}{0.51,0.55,0.55}
\xdefinecolor{azure}{rgb}{0.94,1.00,1.00}
\xdefinecolor{beige}{rgb}{0.96,0.96,0.86}
\xdefinecolor{bisque1}{rgb}{1.00,0.89,0.77}
\xdefinecolor{bisque2}{rgb}{0.93,0.84,0.72}
\xdefinecolor{bisque3}{rgb}{0.80,0.72,0.62}
\xdefinecolor{bisque4}{rgb}{0.55,0.49,0.42}
\xdefinecolor{bisque}{rgb}{1.00,0.89,0.77}
\xdefinecolor{black}{rgb}{0.00,0.00,0.00}
\xdefinecolor{blanchedalmond}{rgb}{1.00,0.92,0.80}
\xdefinecolor{blue1}{rgb}{0.00,0.00,1.00}
\xdefinecolor{blue2}{rgb}{0.00,0.00,0.93}
\xdefinecolor{blue3}{rgb}{0.00,0.00,0.80}
\xdefinecolor{blue4}{rgb}{0.00,0.00,0.55}
\xdefinecolor{blueviolet}{rgb}{0.54,0.17,0.89}
\xdefinecolor{blue}{rgb}{0.00,0.00,1.00}
\xdefinecolor{brown1}{rgb}{1.00,0.25,0.25}
\xdefinecolor{brown2}{rgb}{0.93,0.23,0.23}
\xdefinecolor{brown3}{rgb}{0.80,0.20,0.20}
\xdefinecolor{brown4}{rgb}{0.55,0.14,0.14}
\xdefinecolor{brown}{rgb}{0.65,0.16,0.16}
\xdefinecolor{burlywood1}{rgb}{1.00,0.83,0.61}
\xdefinecolor{burlywood2}{rgb}{0.93,0.77,0.57}
\xdefinecolor{burlywood3}{rgb}{0.80,0.67,0.49}
\xdefinecolor{burlywood4}{rgb}{0.55,0.45,0.33}
\xdefinecolor{burlywood}{rgb}{0.87,0.72,0.53}
\xdefinecolor{cadetblue}{rgb}{0.37,0.62,0.63}
\xdefinecolor{chartreuse1}{rgb}{0.50,1.00,0.00}
\xdefinecolor{chartreuse2}{rgb}{0.46,0.93,0.00}
\xdefinecolor{chartreuse3}{rgb}{0.40,0.80,0.00}
\xdefinecolor{chartreuse4}{rgb}{0.27,0.55,0.00}
\xdefinecolor{chartreuse}{rgb}{0.50,1.00,0.00}
\xdefinecolor{chocolate1}{rgb}{1.00,0.50,0.14}
\xdefinecolor{chocolate2}{rgb}{0.93,0.46,0.13}
\xdefinecolor{chocolate3}{rgb}{0.80,0.40,0.11}
\xdefinecolor{chocolate4}{rgb}{0.55,0.27,0.07}
\xdefinecolor{chocolate}{rgb}{0.82,0.41,0.12}
\xdefinecolor{coral1}{rgb}{1.00,0.45,0.34}
\xdefinecolor{coral2}{rgb}{0.93,0.42,0.31}
\xdefinecolor{coral3}{rgb}{0.80,0.36,0.27}
\xdefinecolor{coral4}{rgb}{0.55,0.24,0.18}
\xdefinecolor{coral}{rgb}{1.00,0.50,0.31}
\xdefinecolor{cornflowerblue}{rgb}{0.39,0.58,0.93}
\xdefinecolor{cornsilk1}{rgb}{1.00,0.97,0.86}
\xdefinecolor{cornsilk2}{rgb}{0.93,0.91,0.80}
\xdefinecolor{cornsilk3}{rgb}{0.80,0.78,0.69}
\xdefinecolor{cornsilk4}{rgb}{0.55,0.53,0.47}
\xdefinecolor{cornsilk}{rgb}{1.00,0.97,0.86}
\xdefinecolor{cyan1}{rgb}{0.00,1.00,1.00}
\xdefinecolor{cyan2}{rgb}{0.00,0.93,0.93}
\xdefinecolor{cyan3}{rgb}{0.00,0.80,0.80}
\xdefinecolor{cyan4}{rgb}{0.00,0.55,0.55}
\xdefinecolor{cyan}{rgb}{0.00,1.00,1.00}
\xdefinecolor{darkblue}{rgb}{0.00,0.00,0.55}
\xdefinecolor{darkcyan}{rgb}{0.00,0.55,0.55}
\xdefinecolor{darkgoldenrod}{rgb}{0.72,0.53,0.04}
\xdefinecolor{darkgray}{rgb}{0.66,0.66,0.66}
\xdefinecolor{darkgreen}{rgb}{0.00,0.39,0.00}
\xdefinecolor{darkgrey}{rgb}{0.66,0.66,0.66}
\xdefinecolor{darkkhaki}{rgb}{0.74,0.72,0.42}
\xdefinecolor{darkmagenta}{rgb}{0.55,0.00,0.55}
\xdefinecolor{darkolive}{rgb}{0.33,0.42,0.18}
\xdefinecolor{darkorange}{rgb}{1.00,0.55,0.00}
\xdefinecolor{darkorchid}{rgb}{0.60,0.20,0.80}
\xdefinecolor{darkred}{rgb}{0.55,0.00,0.00}
\xdefinecolor{darksalmon}{rgb}{0.91,0.59,0.48}
\xdefinecolor{darksea}{rgb}{0.56,0.74,0.56}
\xdefinecolor{darkslate}{rgb}{0.18,0.31,0.31}
\xdefinecolor{darkslate}{rgb}{0.18,0.31,0.31}
\xdefinecolor{darkslate}{rgb}{0.28,0.24,0.55}
\xdefinecolor{darkturquoise}{rgb}{0.00,0.81,0.82}
\xdefinecolor{darkviolet}{rgb}{0.58,0.00,0.83}
\xdefinecolor{deeppink}{rgb}{1.00,0.08,0.58}
\xdefinecolor{deepsky}{rgb}{0.00,0.75,1.00}
\xdefinecolor{dimgray}{rgb}{0.41,0.41,0.41}
\xdefinecolor{dimgrey}{rgb}{0.41,0.41,0.41}
\xdefinecolor{dodgerblue}{rgb}{0.12,0.56,1.00}
\xdefinecolor{firebrick1}{rgb}{1.00,0.19,0.19}
\xdefinecolor{firebrick2}{rgb}{0.93,0.17,0.17}
\xdefinecolor{firebrick3}{rgb}{0.80,0.15,0.15}
\xdefinecolor{firebrick4}{rgb}{0.55,0.10,0.10}
\xdefinecolor{firebrick}{rgb}{0.70,0.13,0.13}
\xdefinecolor{floralwhite}{rgb}{1.00,0.98,0.94}
\xdefinecolor{forestgreen}{rgb}{0.13,0.55,0.13}
\xdefinecolor{gainsboro}{rgb}{0.86,0.86,0.86}
\xdefinecolor{ghostwhite}{rgb}{0.97,0.97,1.00}
\xdefinecolor{gold1}{rgb}{1.00,0.84,0.00}
\xdefinecolor{gold2}{rgb}{0.93,0.79,0.00}
\xdefinecolor{gold3}{rgb}{0.80,0.68,0.00}
\xdefinecolor{gold4}{rgb}{0.55,0.46,0.00}
\xdefinecolor{goldenrod1}{rgb}{1.00,0.76,0.15}
\xdefinecolor{goldenrod2}{rgb}{0.93,0.71,0.13}
\xdefinecolor{goldenrod3}{rgb}{0.80,0.61,0.11}
\xdefinecolor{goldenrod4}{rgb}{0.55,0.41,0.08}
\xdefinecolor{goldenrod}{rgb}{0.85,0.65,0.13}
\xdefinecolor{gold}{rgb}{1.00,0.84,0.00}
\xdefinecolor{gray0}{rgb}{0.00,0.00,0.00}
\xdefinecolor{gray100}{rgb}{1.00,1.00,1.00}
\xdefinecolor{gray10}{rgb}{0.10,0.10,0.10}
\xdefinecolor{gray11}{rgb}{0.11,0.11,0.11}
\xdefinecolor{gray12}{rgb}{0.12,0.12,0.12}
\xdefinecolor{gray13}{rgb}{0.13,0.13,0.13}
\xdefinecolor{gray14}{rgb}{0.14,0.14,0.14}
\xdefinecolor{gray15}{rgb}{0.15,0.15,0.15}
\xdefinecolor{gray16}{rgb}{0.16,0.16,0.16}
\xdefinecolor{gray17}{rgb}{0.17,0.17,0.17}
\xdefinecolor{gray18}{rgb}{0.18,0.18,0.18}
\xdefinecolor{gray19}{rgb}{0.19,0.19,0.19}
\xdefinecolor{gray1}{rgb}{0.01,0.01,0.01}
\xdefinecolor{gray20}{rgb}{0.20,0.20,0.20}
\xdefinecolor{gray21}{rgb}{0.21,0.21,0.21}
\xdefinecolor{gray22}{rgb}{0.22,0.22,0.22}
\xdefinecolor{gray23}{rgb}{0.23,0.23,0.23}
\xdefinecolor{gray24}{rgb}{0.24,0.24,0.24}
\xdefinecolor{gray25}{rgb}{0.25,0.25,0.25}
\xdefinecolor{gray26}{rgb}{0.26,0.26,0.26}
\xdefinecolor{gray27}{rgb}{0.27,0.27,0.27}
\xdefinecolor{gray28}{rgb}{0.28,0.28,0.28}
\xdefinecolor{gray29}{rgb}{0.29,0.29,0.29}
\xdefinecolor{gray2}{rgb}{0.02,0.02,0.02}
\xdefinecolor{gray30}{rgb}{0.30,0.30,0.30}
\xdefinecolor{gray31}{rgb}{0.31,0.31,0.31}
\xdefinecolor{gray32}{rgb}{0.32,0.32,0.32}
\xdefinecolor{gray33}{rgb}{0.33,0.33,0.33}
\xdefinecolor{gray34}{rgb}{0.34,0.34,0.34}
\xdefinecolor{gray35}{rgb}{0.35,0.35,0.35}
\xdefinecolor{gray36}{rgb}{0.36,0.36,0.36}
\xdefinecolor{gray37}{rgb}{0.37,0.37,0.37}
\xdefinecolor{gray38}{rgb}{0.38,0.38,0.38}
\xdefinecolor{gray39}{rgb}{0.39,0.39,0.39}
\xdefinecolor{gray3}{rgb}{0.03,0.03,0.03}
\xdefinecolor{gray40}{rgb}{0.40,0.40,0.40}
\xdefinecolor{gray41}{rgb}{0.41,0.41,0.41}
\xdefinecolor{gray42}{rgb}{0.42,0.42,0.42}
\xdefinecolor{gray43}{rgb}{0.43,0.43,0.43}
\xdefinecolor{gray44}{rgb}{0.44,0.44,0.44}
\xdefinecolor{gray45}{rgb}{0.45,0.45,0.45}
\xdefinecolor{gray46}{rgb}{0.46,0.46,0.46}
\xdefinecolor{gray47}{rgb}{0.47,0.47,0.47}
\xdefinecolor{gray48}{rgb}{0.48,0.48,0.48}
\xdefinecolor{gray49}{rgb}{0.49,0.49,0.49}
\xdefinecolor{gray4}{rgb}{0.04,0.04,0.04}
\xdefinecolor{gray50}{rgb}{0.50,0.50,0.50}
\xdefinecolor{gray51}{rgb}{0.51,0.51,0.51}
\xdefinecolor{gray52}{rgb}{0.52,0.52,0.52}
\xdefinecolor{gray53}{rgb}{0.53,0.53,0.53}
\xdefinecolor{gray54}{rgb}{0.54,0.54,0.54}
\xdefinecolor{gray55}{rgb}{0.55,0.55,0.55}
\xdefinecolor{gray56}{rgb}{0.56,0.56,0.56}
\xdefinecolor{gray57}{rgb}{0.57,0.57,0.57}
\xdefinecolor{gray58}{rgb}{0.58,0.58,0.58}
\xdefinecolor{gray59}{rgb}{0.59,0.59,0.59}
\xdefinecolor{gray5}{rgb}{0.05,0.05,0.05}
\xdefinecolor{gray60}{rgb}{0.60,0.60,0.60}
\xdefinecolor{gray61}{rgb}{0.61,0.61,0.61}
\xdefinecolor{gray62}{rgb}{0.62,0.62,0.62}
\xdefinecolor{gray63}{rgb}{0.63,0.63,0.63}
\xdefinecolor{gray64}{rgb}{0.64,0.64,0.64}
\xdefinecolor{gray65}{rgb}{0.65,0.65,0.65}
\xdefinecolor{gray66}{rgb}{0.66,0.66,0.66}
\xdefinecolor{gray67}{rgb}{0.67,0.67,0.67}
\xdefinecolor{gray68}{rgb}{0.68,0.68,0.68}
\xdefinecolor{gray69}{rgb}{0.69,0.69,0.69}
\xdefinecolor{gray6}{rgb}{0.06,0.06,0.06}
\xdefinecolor{gray70}{rgb}{0.70,0.70,0.70}
\xdefinecolor{gray71}{rgb}{0.71,0.71,0.71}
\xdefinecolor{gray72}{rgb}{0.72,0.72,0.72}
\xdefinecolor{gray73}{rgb}{0.73,0.73,0.73}
\xdefinecolor{gray74}{rgb}{0.74,0.74,0.74}
\xdefinecolor{gray75}{rgb}{0.75,0.75,0.75}
\xdefinecolor{gray76}{rgb}{0.76,0.76,0.76}
\xdefinecolor{gray77}{rgb}{0.77,0.77,0.77}
\xdefinecolor{gray78}{rgb}{0.78,0.78,0.78}
\xdefinecolor{gray79}{rgb}{0.79,0.79,0.79}
\xdefinecolor{gray7}{rgb}{0.07,0.07,0.07}
\xdefinecolor{gray80}{rgb}{0.80,0.80,0.80}
\xdefinecolor{gray81}{rgb}{0.81,0.81,0.81}
\xdefinecolor{gray82}{rgb}{0.82,0.82,0.82}
\xdefinecolor{gray83}{rgb}{0.83,0.83,0.83}
\xdefinecolor{gray84}{rgb}{0.84,0.84,0.84}
\xdefinecolor{gray85}{rgb}{0.85,0.85,0.85}
\xdefinecolor{gray86}{rgb}{0.86,0.86,0.86}
\xdefinecolor{gray87}{rgb}{0.87,0.87,0.87}
\xdefinecolor{gray88}{rgb}{0.88,0.88,0.88}
\xdefinecolor{gray89}{rgb}{0.89,0.89,0.89}
\xdefinecolor{gray8}{rgb}{0.08,0.08,0.08}
\xdefinecolor{gray90}{rgb}{0.90,0.90,0.90}
\xdefinecolor{gray91}{rgb}{0.91,0.91,0.91}
\xdefinecolor{gray92}{rgb}{0.92,0.92,0.92}
\xdefinecolor{gray93}{rgb}{0.93,0.93,0.93}
\xdefinecolor{gray94}{rgb}{0.94,0.94,0.94}
\xdefinecolor{gray95}{rgb}{0.95,0.95,0.95}
\xdefinecolor{gray96}{rgb}{0.96,0.96,0.96}
\xdefinecolor{gray97}{rgb}{0.97,0.97,0.97}
\xdefinecolor{gray98}{rgb}{0.98,0.98,0.98}
\xdefinecolor{gray99}{rgb}{0.99,0.99,0.99}
\xdefinecolor{gray9}{rgb}{0.09,0.09,0.09}
\xdefinecolor{gray}{rgb}{0.75,0.75,0.75}
\xdefinecolor{green1}{rgb}{0.00,1.00,0.00}
\xdefinecolor{green2}{rgb}{0.00,0.93,0.00}
\xdefinecolor{green3}{rgb}{0.00,0.80,0.00}
\xdefinecolor{green4}{rgb}{0.00,0.55,0.00}
\xdefinecolor{greenyellow}{rgb}{0.68,1.00,0.18}
\xdefinecolor{green}{rgb}{0.00,1.00,0.00}
\xdefinecolor{grey0}{rgb}{0.00,0.00,0.00}
\xdefinecolor{grey100}{rgb}{1.00,1.00,1.00}
\xdefinecolor{grey10}{rgb}{0.10,0.10,0.10}
\xdefinecolor{grey11}{rgb}{0.11,0.11,0.11}
\xdefinecolor{grey12}{rgb}{0.12,0.12,0.12}
\xdefinecolor{grey13}{rgb}{0.13,0.13,0.13}
\xdefinecolor{grey14}{rgb}{0.14,0.14,0.14}
\xdefinecolor{grey15}{rgb}{0.15,0.15,0.15}
\xdefinecolor{grey16}{rgb}{0.16,0.16,0.16}
\xdefinecolor{grey17}{rgb}{0.17,0.17,0.17}
\xdefinecolor{grey18}{rgb}{0.18,0.18,0.18}
\xdefinecolor{grey19}{rgb}{0.19,0.19,0.19}
\xdefinecolor{grey1}{rgb}{0.01,0.01,0.01}
\xdefinecolor{grey20}{rgb}{0.20,0.20,0.20}
\xdefinecolor{grey21}{rgb}{0.21,0.21,0.21}
\xdefinecolor{grey22}{rgb}{0.22,0.22,0.22}
\xdefinecolor{grey23}{rgb}{0.23,0.23,0.23}
\xdefinecolor{grey24}{rgb}{0.24,0.24,0.24}
\xdefinecolor{grey25}{rgb}{0.25,0.25,0.25}
\xdefinecolor{grey26}{rgb}{0.26,0.26,0.26}
\xdefinecolor{grey27}{rgb}{0.27,0.27,0.27}
\xdefinecolor{grey28}{rgb}{0.28,0.28,0.28}
\xdefinecolor{grey29}{rgb}{0.29,0.29,0.29}
\xdefinecolor{grey2}{rgb}{0.02,0.02,0.02}
\xdefinecolor{grey30}{rgb}{0.30,0.30,0.30}
\xdefinecolor{grey31}{rgb}{0.31,0.31,0.31}
\xdefinecolor{grey32}{rgb}{0.32,0.32,0.32}
\xdefinecolor{grey33}{rgb}{0.33,0.33,0.33}
\xdefinecolor{grey34}{rgb}{0.34,0.34,0.34}
\xdefinecolor{grey35}{rgb}{0.35,0.35,0.35}
\xdefinecolor{grey36}{rgb}{0.36,0.36,0.36}
\xdefinecolor{grey37}{rgb}{0.37,0.37,0.37}
\xdefinecolor{grey38}{rgb}{0.38,0.38,0.38}
\xdefinecolor{grey39}{rgb}{0.39,0.39,0.39}
\xdefinecolor{grey3}{rgb}{0.03,0.03,0.03}
\xdefinecolor{grey40}{rgb}{0.40,0.40,0.40}
\xdefinecolor{grey41}{rgb}{0.41,0.41,0.41}
\xdefinecolor{grey42}{rgb}{0.42,0.42,0.42}
\xdefinecolor{grey43}{rgb}{0.43,0.43,0.43}
\xdefinecolor{grey44}{rgb}{0.44,0.44,0.44}
\xdefinecolor{grey45}{rgb}{0.45,0.45,0.45}
\xdefinecolor{grey46}{rgb}{0.46,0.46,0.46}
\xdefinecolor{grey47}{rgb}{0.47,0.47,0.47}
\xdefinecolor{grey48}{rgb}{0.48,0.48,0.48}
\xdefinecolor{grey49}{rgb}{0.49,0.49,0.49}
\xdefinecolor{grey4}{rgb}{0.04,0.04,0.04}
\xdefinecolor{grey50}{rgb}{0.50,0.50,0.50}
\xdefinecolor{grey51}{rgb}{0.51,0.51,0.51}
\xdefinecolor{grey52}{rgb}{0.52,0.52,0.52}
\xdefinecolor{grey53}{rgb}{0.53,0.53,0.53}
\xdefinecolor{grey54}{rgb}{0.54,0.54,0.54}
\xdefinecolor{grey55}{rgb}{0.55,0.55,0.55}
\xdefinecolor{grey56}{rgb}{0.56,0.56,0.56}
\xdefinecolor{grey57}{rgb}{0.57,0.57,0.57}
\xdefinecolor{grey58}{rgb}{0.58,0.58,0.58}
\xdefinecolor{grey59}{rgb}{0.59,0.59,0.59}
\xdefinecolor{grey5}{rgb}{0.05,0.05,0.05}
\xdefinecolor{grey60}{rgb}{0.60,0.60,0.60}
\xdefinecolor{grey61}{rgb}{0.61,0.61,0.61}
\xdefinecolor{grey62}{rgb}{0.62,0.62,0.62}
\xdefinecolor{grey63}{rgb}{0.63,0.63,0.63}
\xdefinecolor{grey64}{rgb}{0.64,0.64,0.64}
\xdefinecolor{grey65}{rgb}{0.65,0.65,0.65}
\xdefinecolor{grey66}{rgb}{0.66,0.66,0.66}
\xdefinecolor{grey67}{rgb}{0.67,0.67,0.67}
\xdefinecolor{grey68}{rgb}{0.68,0.68,0.68}
\xdefinecolor{grey69}{rgb}{0.69,0.69,0.69}
\xdefinecolor{grey6}{rgb}{0.06,0.06,0.06}
\xdefinecolor{grey70}{rgb}{0.70,0.70,0.70}
\xdefinecolor{grey71}{rgb}{0.71,0.71,0.71}
\xdefinecolor{grey72}{rgb}{0.72,0.72,0.72}
\xdefinecolor{grey73}{rgb}{0.73,0.73,0.73}
\xdefinecolor{grey74}{rgb}{0.74,0.74,0.74}
\xdefinecolor{grey75}{rgb}{0.75,0.75,0.75}
\xdefinecolor{grey76}{rgb}{0.76,0.76,0.76}
\xdefinecolor{grey77}{rgb}{0.77,0.77,0.77}
\xdefinecolor{grey78}{rgb}{0.78,0.78,0.78}
\xdefinecolor{grey79}{rgb}{0.79,0.79,0.79}
\xdefinecolor{grey7}{rgb}{0.07,0.07,0.07}
\xdefinecolor{grey80}{rgb}{0.80,0.80,0.80}
\xdefinecolor{grey81}{rgb}{0.81,0.81,0.81}
\xdefinecolor{grey82}{rgb}{0.82,0.82,0.82}
\xdefinecolor{grey83}{rgb}{0.83,0.83,0.83}
\xdefinecolor{grey84}{rgb}{0.84,0.84,0.84}
\xdefinecolor{grey85}{rgb}{0.85,0.85,0.85}
\xdefinecolor{grey86}{rgb}{0.86,0.86,0.86}
\xdefinecolor{grey87}{rgb}{0.87,0.87,0.87}
\xdefinecolor{grey88}{rgb}{0.88,0.88,0.88}
\xdefinecolor{grey89}{rgb}{0.89,0.89,0.89}
\xdefinecolor{grey8}{rgb}{0.08,0.08,0.08}
\xdefinecolor{grey90}{rgb}{0.90,0.90,0.90}
\xdefinecolor{grey91}{rgb}{0.91,0.91,0.91}
\xdefinecolor{grey92}{rgb}{0.92,0.92,0.92}
\xdefinecolor{grey93}{rgb}{0.93,0.93,0.93}
\xdefinecolor{grey94}{rgb}{0.94,0.94,0.94}
\xdefinecolor{grey95}{rgb}{0.95,0.95,0.95}
\xdefinecolor{grey96}{rgb}{0.96,0.96,0.96}
\xdefinecolor{grey97}{rgb}{0.97,0.97,0.97}
\xdefinecolor{grey98}{rgb}{0.98,0.98,0.98}
\xdefinecolor{grey99}{rgb}{0.99,0.99,0.99}
\xdefinecolor{grey9}{rgb}{0.09,0.09,0.09}
\xdefinecolor{grey}{rgb}{0.75,0.75,0.75}
\xdefinecolor{honeydew1}{rgb}{0.94,1.00,0.94}
\xdefinecolor{honeydew2}{rgb}{0.88,0.93,0.88}
\xdefinecolor{honeydew3}{rgb}{0.76,0.80,0.76}
\xdefinecolor{honeydew4}{rgb}{0.51,0.55,0.51}
\xdefinecolor{honeydew}{rgb}{0.94,1.00,0.94}
\xdefinecolor{hotpink}{rgb}{1.00,0.41,0.71}
\xdefinecolor{indianred}{rgb}{0.80,0.36,0.36}
\xdefinecolor{ivory1}{rgb}{1.00,1.00,0.94}
\xdefinecolor{ivory2}{rgb}{0.93,0.93,0.88}
\xdefinecolor{ivory3}{rgb}{0.80,0.80,0.76}
\xdefinecolor{ivory4}{rgb}{0.55,0.55,0.51}
\xdefinecolor{ivory}{rgb}{1.00,1.00,0.94}
\xdefinecolor{khaki1}{rgb}{1.00,0.96,0.56}
\xdefinecolor{khaki2}{rgb}{0.93,0.90,0.52}
\xdefinecolor{khaki3}{rgb}{0.80,0.78,0.45}
\xdefinecolor{khaki4}{rgb}{0.55,0.53,0.31}
\xdefinecolor{khaki}{rgb}{0.94,0.90,0.55}
\xdefinecolor{lavenderblush}{rgb}{1.00,0.94,0.96}
\xdefinecolor{lavender}{rgb}{0.90,0.90,0.98}
\xdefinecolor{lawngreen}{rgb}{0.49,0.99,0.00}
\xdefinecolor{lemonchiffon}{rgb}{1.00,0.98,0.80}
\xdefinecolor{lightblue}{rgb}{0.68,0.85,0.90}
\xdefinecolor{lightcoral}{rgb}{0.94,0.50,0.50}
\xdefinecolor{lightcyan}{rgb}{0.88,1.00,1.00}
\xdefinecolor{lightgoldenrod}{rgb}{0.93,0.87,0.51}
\xdefinecolor{lightgoldenrod}{rgb}{0.98,0.98,0.82}
\xdefinecolor{lightgray}{rgb}{0.83,0.83,0.83}
\xdefinecolor{lightgreen}{rgb}{0.56,0.93,0.56}
\xdefinecolor{lightgrey}{rgb}{0.83,0.83,0.83}
\xdefinecolor{lightpink}{rgb}{1.00,0.71,0.76}
\xdefinecolor{lightsalmon}{rgb}{1.00,0.63,0.48}
\xdefinecolor{lightsea}{rgb}{0.13,0.70,0.67}
\xdefinecolor{lightsky}{rgb}{0.53,0.81,0.98}
\xdefinecolor{lightslate}{rgb}{0.47,0.53,0.60}
\xdefinecolor{lightslate}{rgb}{0.47,0.53,0.60}
\xdefinecolor{lightslate}{rgb}{0.52,0.44,1.00}
\xdefinecolor{lightsteel}{rgb}{0.69,0.77,0.87}
\xdefinecolor{lightyellow}{rgb}{1.00,1.00,0.88}
\xdefinecolor{limegreen}{rgb}{0.20,0.80,0.20}
\xdefinecolor{linen}{rgb}{0.98,0.94,0.90}
\xdefinecolor{magenta1}{rgb}{1.00,0.00,1.00}
\xdefinecolor{magenta2}{rgb}{0.93,0.00,0.93}
\xdefinecolor{magenta3}{rgb}{0.80,0.00,0.80}
\xdefinecolor{magenta4}{rgb}{0.55,0.00,0.55}
\xdefinecolor{magenta}{rgb}{1.00,0.00,1.00}
\xdefinecolor{maroon1}{rgb}{1.00,0.20,0.70}
\xdefinecolor{maroon2}{rgb}{0.93,0.19,0.65}
\xdefinecolor{maroon3}{rgb}{0.80,0.16,0.56}
\xdefinecolor{maroon4}{rgb}{0.55,0.11,0.38}
\xdefinecolor{maroon}{rgb}{0.69,0.19,0.38}
\xdefinecolor{mediumaquamarine}{rgb}{0.40,0.80,0.67}
\xdefinecolor{mediumblue}{rgb}{0.00,0.00,0.80}
\xdefinecolor{mediumorchid}{rgb}{0.73,0.33,0.83}
\xdefinecolor{mediumpurple}{rgb}{0.58,0.44,0.86}
\xdefinecolor{mediumsea}{rgb}{0.24,0.70,0.44}
\xdefinecolor{mediumslate}{rgb}{0.48,0.41,0.93}
\xdefinecolor{mediumspring}{rgb}{0.00,0.98,0.60}
\xdefinecolor{mediumturquoise}{rgb}{0.28,0.82,0.80}
\xdefinecolor{mediumviolet}{rgb}{0.78,0.08,0.52}
\xdefinecolor{midnightblue}{rgb}{0.10,0.10,0.44}
\xdefinecolor{mintcream}{rgb}{0.96,1.00,0.98}
\xdefinecolor{mistyrose}{rgb}{1.00,0.89,0.88}
\xdefinecolor{moccasin}{rgb}{1.00,0.89,0.71}
\xdefinecolor{navajowhite}{rgb}{1.00,0.87,0.68}
\xdefinecolor{navyblue}{rgb}{0.00,0.00,0.50}
\xdefinecolor{navy}{rgb}{0.00,0.00,0.50}
\xdefinecolor{oldlace}{rgb}{0.99,0.96,0.90}
\xdefinecolor{olivedrab}{rgb}{0.42,0.56,0.14}
\xdefinecolor{orange1}{rgb}{1.00,0.65,0.00}
\xdefinecolor{orange2}{rgb}{0.93,0.60,0.00}
\xdefinecolor{orange3}{rgb}{0.80,0.52,0.00}
\xdefinecolor{orange4}{rgb}{0.55,0.35,0.00}
\xdefinecolor{orangered}{rgb}{1.00,0.27,0.00}
\xdefinecolor{orange}{rgb}{1.00,0.65,0.00}
\xdefinecolor{orchid1}{rgb}{1.00,0.51,0.98}
\xdefinecolor{orchid2}{rgb}{0.93,0.48,0.91}
\xdefinecolor{orchid3}{rgb}{0.80,0.41,0.79}
\xdefinecolor{orchid4}{rgb}{0.55,0.28,0.54}
\xdefinecolor{orchid}{rgb}{0.85,0.44,0.84}
\xdefinecolor{palegoldenrod}{rgb}{0.93,0.91,0.67}
\xdefinecolor{palegreen}{rgb}{0.60,0.98,0.60}
\xdefinecolor{paleturquoise}{rgb}{0.69,0.93,0.93}
\xdefinecolor{paleviolet}{rgb}{0.86,0.44,0.58}
\xdefinecolor{papayawhip}{rgb}{1.00,0.94,0.84}
\xdefinecolor{peachpuff}{rgb}{1.00,0.85,0.73}
\xdefinecolor{peru}{rgb}{0.80,0.52,0.25}
\xdefinecolor{pink1}{rgb}{1.00,0.71,0.77}
\xdefinecolor{pink2}{rgb}{0.93,0.66,0.72}
\xdefinecolor{pink3}{rgb}{0.80,0.57,0.62}
\xdefinecolor{pink4}{rgb}{0.55,0.39,0.42}
\xdefinecolor{pink}{rgb}{1.00,0.75,0.80}
\xdefinecolor{plum1}{rgb}{1.00,0.73,1.00}
\xdefinecolor{plum2}{rgb}{0.93,0.68,0.93}
\xdefinecolor{plum3}{rgb}{0.80,0.59,0.80}
\xdefinecolor{plum4}{rgb}{0.55,0.40,0.55}
\xdefinecolor{plum}{rgb}{0.87,0.63,0.87}
\xdefinecolor{powderblue}{rgb}{0.69,0.88,0.90}
\xdefinecolor{purple1}{rgb}{0.61,0.19,1.00}
\xdefinecolor{purple2}{rgb}{0.57,0.17,0.93}
\xdefinecolor{purple3}{rgb}{0.49,0.15,0.80}
\xdefinecolor{purple4}{rgb}{0.33,0.10,0.55}
\xdefinecolor{purple}{rgb}{0.63,0.13,0.94}
\xdefinecolor{red1}{rgb}{1.00,0.00,0.00}
\xdefinecolor{red2}{rgb}{0.93,0.00,0.00}
\xdefinecolor{red3}{rgb}{0.80,0.00,0.00}
\xdefinecolor{red4}{rgb}{0.55,0.00,0.00}
\xdefinecolor{red}{rgb}{1.00,0.00,0.00}
\xdefinecolor{rosybrown}{rgb}{0.74,0.56,0.56}
\xdefinecolor{royalblue}{rgb}{0.25,0.41,0.88}
\xdefinecolor{saddlebrown}{rgb}{0.55,0.27,0.07}
\xdefinecolor{salmon1}{rgb}{1.00,0.55,0.41}
\xdefinecolor{salmon2}{rgb}{0.93,0.51,0.38}
\xdefinecolor{salmon3}{rgb}{0.80,0.44,0.33}
\xdefinecolor{salmon4}{rgb}{0.55,0.30,0.22}
\xdefinecolor{salmon}{rgb}{0.98,0.50,0.45}
\xdefinecolor{sandybrown}{rgb}{0.96,0.64,0.38}
\xdefinecolor{seagreen}{rgb}{0.18,0.55,0.34}
\xdefinecolor{seashell1}{rgb}{1.00,0.96,0.93}
\xdefinecolor{seashell2}{rgb}{0.93,0.90,0.87}
\xdefinecolor{seashell3}{rgb}{0.80,0.77,0.75}
\xdefinecolor{seashell4}{rgb}{0.55,0.53,0.51}
\xdefinecolor{seashell}{rgb}{1.00,0.96,0.93}
\xdefinecolor{sienna1}{rgb}{1.00,0.51,0.28}
\xdefinecolor{sienna2}{rgb}{0.93,0.47,0.26}
\xdefinecolor{sienna3}{rgb}{0.80,0.41,0.22}
\xdefinecolor{sienna4}{rgb}{0.55,0.28,0.15}
\xdefinecolor{sienna}{rgb}{0.63,0.32,0.18}
\xdefinecolor{skyblue}{rgb}{0.53,0.81,0.92}
\xdefinecolor{slateblue}{rgb}{0.42,0.35,0.80}
\xdefinecolor{slategray}{rgb}{0.44,0.50,0.56}
\xdefinecolor{slategrey}{rgb}{0.44,0.50,0.56}
\xdefinecolor{snow1}{rgb}{1.00,0.98,0.98}
\xdefinecolor{snow2}{rgb}{0.93,0.91,0.91}
\xdefinecolor{snow3}{rgb}{0.80,0.79,0.79}
\xdefinecolor{snow4}{rgb}{0.55,0.54,0.54}
\xdefinecolor{snow}{rgb}{1.00,0.98,0.98}
\xdefinecolor{springgreen}{rgb}{0.00,1.00,0.50}
\xdefinecolor{steelblue}{rgb}{0.27,0.51,0.71}
\xdefinecolor{tan1}{rgb}{1.00,0.65,0.31}
\xdefinecolor{tan2}{rgb}{0.93,0.60,0.29}
\xdefinecolor{tan3}{rgb}{0.80,0.52,0.25}
\xdefinecolor{tan4}{rgb}{0.55,0.35,0.17}
\xdefinecolor{tan}{rgb}{0.82,0.71,0.55}
\xdefinecolor{thistle1}{rgb}{1.00,0.88,1.00}
\xdefinecolor{thistle2}{rgb}{0.93,0.82,0.93}
\xdefinecolor{thistle3}{rgb}{0.80,0.71,0.80}
\xdefinecolor{thistle4}{rgb}{0.55,0.48,0.55}
\xdefinecolor{thistle}{rgb}{0.85,0.75,0.85}
\xdefinecolor{tomato1}{rgb}{1.00,0.39,0.28}
\xdefinecolor{tomato2}{rgb}{0.93,0.36,0.26}
\xdefinecolor{tomato3}{rgb}{0.80,0.31,0.22}
\xdefinecolor{tomato4}{rgb}{0.55,0.21,0.15}
\xdefinecolor{tomato}{rgb}{1.00,0.39,0.28}
\xdefinecolor{turquoise1}{rgb}{0.00,0.96,1.00}
\xdefinecolor{turquoise2}{rgb}{0.00,0.90,0.93}
\xdefinecolor{turquoise3}{rgb}{0.00,0.77,0.80}
\xdefinecolor{turquoise4}{rgb}{0.00,0.53,0.55}
\xdefinecolor{turquoise}{rgb}{0.25,0.88,0.82}
\xdefinecolor{violetred}{rgb}{0.82,0.13,0.56}
\xdefinecolor{violet}{rgb}{0.93,0.51,0.93}
\xdefinecolor{wheat1}{rgb}{1.00,0.91,0.73}
\xdefinecolor{wheat2}{rgb}{0.93,0.85,0.68}
\xdefinecolor{wheat3}{rgb}{0.80,0.73,0.59}
\xdefinecolor{wheat4}{rgb}{0.55,0.49,0.40}
\xdefinecolor{wheat}{rgb}{0.96,0.87,0.70}
\xdefinecolor{whitesmoke}{rgb}{0.96,0.96,0.96}
\xdefinecolor{white}{rgb}{1.00,1.00,1.00}
\xdefinecolor{yellow1}{rgb}{1.00,1.00,0.00}
\xdefinecolor{yellow2}{rgb}{0.93,0.93,0.00}
\xdefinecolor{yellow3}{rgb}{0.80,0.80,0.00}
\xdefinecolor{yellow4}{rgb}{0.55,0.55,0.00}
\xdefinecolor{yellowgreen}{rgb}{0.60,0.80,0.20}
\xdefinecolor{yellow}{rgb}{1.00,1.00,0.00}
\xdefinecolor{mygreen}{rgb}{0,.5,.5}

